Finding Experts in Transformer Models

In this work we study the presence of expert units in pre-trained Transformer Models (TM), and how they impact a model's performance. We define expert units to be neurons that are able to classify a concept with a given average precision, where a concept is represented by a binary set of sentences containing the concept (or not). Leveraging the OneSec dataset (Scarlini et al., 2019), we compile a dataset of 1641 concepts that allows diverse expert units in TM to be discovered. We show that expert units are important in several ways: (1) The presence of expert units is correlated ($r^2=0.833$) with the generalization power of TM, which allows ranking TM without requiring fine-tuning on suites of downstream tasks. We further propose an empirical method to decide how accurate such experts should be to evaluate generalization. (2) The overlap of top experts between concepts provides a sensible way to quantify concept co-learning, which can be used for explainability of unknown concepts. (3) We show how to self-condition off-the-shelf pre-trained language models to generate text with a given concept by forcing the top experts to be active, without requiring re-training the model or using additional parameters.

==> sections/results.tex <==
\begin{figure*}[h]
  \centering
%\subfigure{\includegraphics[width=0.4\textwidth]{images/gpt2-bert-large-distr-bars.pdf}}      
\begin{subfigure}[b]{\textwidth}
    \includegraphics[width=0.99\textwidth]{images/gpt2-roberta-large-distr-bars-all-nums.pdf}
  \end{subfigure}
 
    \caption{
  %Left: $\mmap$ as a function of the model size for different architectures. The measured $\mmap$ decreases linearly with the model size (note that the vertical axis is in log scale). Right: 
  Number of acquired concepts $(\gamma = 0.95)$ per layer type  for model  GPT2-L (I, II) and  RoBERTa-L (III, IV). Shallow layers acquire more \textit{sense} concepts than deep layers, such effect being emphasized in GPT2-L. This behavior is similar to the one observed by \citep{Bau:ICLR:2019} for image GANs. We further observe that B layers acquire 3.5x more concepts than layers A. Layers Aproj and Bproj acquire very few concepts, suggesting that the expanding layers (A, B) in the Transformer block (\fig\ref{fig:transformer_schema}) are more prone to learn concepts. \textit{Homograph} concepts (II, IV) are spread across the layers,  few being detected in the first Transformer blocks. }\label{fig:concept_distribution}
\end{figure*}

\section{Experimental results}
\label{sec:results}

All of the pre-trained models evaluated are obtained from the \href{https://huggingface.co/transformers/}{Huggingface Transformers repository} \citep{Wolf:ARXIV:2019}, version 2.1.1.
More precisely, we analyze\footnote{The corresponding names in the transformers repository are: \texttt{bert-base/large-cased, roberta-base/large/large-mnli, distilbert-base-uncased, gpt2-$\emptyset$/medium/large} and \texttt{xlm-mlm-en-2048}.}: BERT-B/L \citep{Devlin:NAACL:2018}, RoBERTa-S/L/Lm \citep{Liu:NAACL:2019}, DistilBERT \citep{Sanh:ARXIV:2019}, GPT2-S/M/L \citep{Radford:ARXIV:2019} and XLM \citep{Lample:ARXIV:2019}. The sentences are tokenized using the default settings in the repository.


\subsection{Concept distribution}

The distribution of acquired concepts per layer type is shown in \fig\ref{fig:concept_distribution}, for models GPT2-L (I, II) and RoBERTa-L (III, IV).
A concept is considered acquired in a layer  $\ell$ if $\exists\, \ap_c^{(k,\ell)} \geq \gamma$. 
In this experiment, we use $\gamma=0.95$ for visualization purposes, $\gstar$ being too restrictive.
% the differences between layer types, since using $\gstar$ is very restrictive and many layers would not detect any concept. 

%This observation is aligned with the results shown in \citep{Bau:ICLR:2019} for image GANs, suggesting that generative models (such as GPT2) learn concepts in the early layers to compose the data, and still have degrees of freedom to modify it in subsequent layers. 
 We observe that shallow layers in \TM accumulate more concepts than deep layers. Within the Transformer blocks (see \fig\ref{fig:transformer_schema}) in GPT2-L, layers of type B acquire about 3.5x more concepts than layers A and more than 10x than layers Aproj and Bproj. This suggests that the expanding layers (A and B) in the Transformer block are better to learn concepts. RoBERTa-L produces a similar distribution of concepts, with layers A and B accumulating most of the concepts. Compared to GPT2-L, RoBERTa-L has a smaller drop in the number of concepts from shallow to deep layers. GPT2-L is a generative model composed of Transformer decoders, while RoBERTa is a stack of encoders. Our results show that generative architectures in NLP tend to accumulate concepts early in the model. Such an observation was reported  by \citep{Bau:ICLR:2019} in the image GAN domain, but to the best of our knowledge we report the first observation of this phenomenon in the NLP domain. 
%Our results suggest that generative models in the NLP domain (such as GPT2) learn concepts in the early layers to start composing the data, and still have degrees of freedom to modify it and add detail in subsequent layers. 
Refer to \appref\ref{app:concept_distribution} for results on other models.

%\tab
%\begin{itemize}
%\item Number of responsible units per concept (some selected concepts, can't show them all)
%\item Percentage of model unused wrt. our dataset.
%\item Caption: Total number of responsible units (at a $\map > 0.95$ for some concepts, and the percentage wrt. the total number of neurons analyzed. Note the extremely low number of neurons dedicated to a concept.  
%\end{itemize}








\subsection{Concept co-learning results}
\label{sec:colearning_results}
In \tabref\ref{tab:knn_chair}, we show that concepts with related senses present a high overlap of top experts, evidencing concept co-learning. 
More precisely,  we show the 5 concepts $v$ with highest overlap $\overlap{q}{v}$ (defined in \eq\eqref{eq:overlap}) with a query concept $q$. The query concepts considered are represented by the same word (chair) but with different WordNet sense (first row of \tabref\ref{tab:knn_chair}). Observe how the top-5 concepts are coherent with the definition of the query. The fact that the \textit{homograph} concept that disambiguates the query appears with high overlap is also interesting. Concept co-learning can be used for explainability: given a concept with unknown definition (\eg failure cases in a dialogue system), the overlapping concepts can help explain it.
%, proving how the model has acquired the sense of the concept in the top 1\% expert units. 
See \appref\ref{app:co_learning} for extended co-learning results.


%We show in \tabref\ref{tab:knn_chair} the top-5 concepts in terms of co-learning overlap $\overlap{q}{v}$ with a query concept $q$, defined in \eq\eqref{eq:overlap}. Two query concepts are considered, represented by the same word (chair) but with different WordNet sense (first row of \tabref\ref{tab:knn_chair}). We observe how the top-5 concepts are coherent with the definition, showing how the model has acquired the sense of the concept in the top 1\% expert units. See \appref\ref{app:co_learning} for extended co-learning results.


\begin{table}[tb]
  \centering
{\fontsize{8}{10} \selectfont
\setlength{\tabcolsep}{1mm}
\begin{tabular}{llc}
\toprule
\shortstack[l]{WordNet definition\\of query} & {Concept} &  $\overlap{{\color{orange}q}}{v}$ \\
\midrule
\multirow{5}{*}[0px]{\shortstack[l]{A seat for one\\person, with a support\\for the back.}}
& {\color{orange}\href{http://wordnetweb.princeton.edu/perl/webwn?s=chair&sub=Search+WordNet&o2=&o0=1&o8=1&o1=1&o7=&o5=&o9=&o6=1&o3=&o4=&h=000000000000}{chair\%1:06:00} (query)}                 &    1.000 \\
& \href{http://wordnetweb.princeton.edu/perl/webwn?o2=&o0=1&o8=1&o1=1&o7=&o5=&o9=&o6=1&o3=&o4=&s=table&h=00000000&j=1#c}{table\%1:06:01}                  &    0.458 \\
& \href{http://wordnetweb.princeton.edu/perl/webwn?s=bed&sub=Search+WordNet&o2=&o0=1&o8=1&o1=1&o7=&o5=&o9=&o6=1&o3=&o4=&h=00000000}{bed\%1:06:00}                     &    0.361 \\
& \href{http://wordnetweb.princeton.edu/perl/webwn?s=cup&sub=Search+WordNet&o2=&o0=1&o8=1&o1=1&o7=&o5=&o9=&o6=1&o3=&o4=&h=0000000000000}{cup\%1:06:00}                     &    0.341 \\
& \href{http://wordnetweb.princeton.edu/perl/webwn?s=table&sub=Search+WordNet&o2=&o0=1&o8=1&o1=1&o7=&o5=&o9=&o6=1&o3=&o4=&h=00000000000}{table\%1:06:01} VS. \href{http://wordnetweb.princeton.edu/perl/webwn?o2=&o0=1&o8=1&o1=1&o7=&o5=&o9=&o6=1&o3=&o4=&s=table&h=00000000&j=1#c}{table\%1:14:00} &    0.336 \\
& \href{http://wordnetweb.princeton.edu/perl/webwn?s=floor&sub=Search+WordNet&o2=&o0=1&o8=1&o1=1&o7=&o5=&o9=&o6=1&o3=&o4=&h=00000000}{floor\%1:06:00}                   &    0.328 \\
\midrule
\multirow{5}{*}[0px]{\shortstack[l]{The position\\of professor.}}
& {\color{orange}\href{http://wordnetweb.princeton.edu/perl/webwn?s=chair&sub=Search+WordNet&o2=&o0=1&o8=1&o1=1&o7=&o5=&o9=&o6=1&o3=&o4=&h=000000000000}{chair\%1:04:00} (query)}                  &    1.000 \\
& \href{http://wordnetweb.princeton.edu/perl/webwn?s=chair&sub=Search+WordNet&o2=&o0=1&o8=1&o1=1&o7=&o5=&o9=&o6=1&o3=&o4=&h=000000000000}{chair\%1:04:00} VS. \href{http://wordnetweb.princeton.edu/perl/webwn?s=chair&sub=Search+WordNet&o2=&o0=1&o8=1&o1=1&o7=&o5=&o9=&o6=1&o3=&o4=&h=000000000000}{chair\%1:06:00} &    0.575 \\
& \href{http://wordnetweb.princeton.edu/perl/webwn?s=fellow&sub=Search+WordNet&o2=&o0=1&o8=1&o1=1&o7=&o5=&o9=&o6=1&o3=&o4=&h=0000000}{fellow\%1:18:02}                  &    0.371 \\
& \href{http://wordnetweb.princeton.edu/perl/webwn?s=director&sub=Search+WordNet&o2=&o0=1&o8=1&o1=1&o7=&o5=&o9=&o6=1&o3=&o4=&h=0000000}{director\%1:18:03}                &    0.297 \\
& \href{http://wordnetweb.princeton.edu/perl/webwn?s=administration&sub=Search+WordNet&o2=&o0=1&o8=1&o1=1&o7=&o5=&o9=&o6=1&o3=&o4=&h=00000}{administration\%1:04:00}          &    0.243 \\
& \href{http://wordnetweb.princeton.edu/perl/webwn?s=member&sub=Search+WordNet&o2=&o0=1&o8=1&o1=1&o7=&o5=&o9=&o6=1&o3=&o4=&h=000000}{member\%1:18:00}                  &    0.241 \\
\bottomrule
\end{tabular}
}
 \caption{
Top-5 concepts in terms of expert overlap $\overlap{{\color{orange}q}}{v}$ (\eq\eqref{eq:overlap}) with a {\color{orange}{query}} concept for RoBERTa-L. The overlap shows the amount of top experts shared by two concepts ${\color{orange}q}$ and $v$. Even if the word representing the concept is the same (chair), the concepts overlapping are different and relate to the actual WordNet definition (click each concept for WordNet link), showing that the model takes the meaning into account. Concepts marked with `VS.' are \textit{homograph} concepts.
 }
  \label{tab:knn_chair}
\end{table}



\begin{table*}[t]
  \centering
{\fontsize{8.5}{8.5} \selectfont
\setlength{\tabcolsep}{1mm}
\begin{tabular}{lp{13.5cm}}
\toprule
K forced &        \hspace{-0mm}{\color{gray}Once upon a time}   {\small$+$} Generated induced for concept \href{\wordnet{bird}}{bird\%1:05:00} (warm-blooded egg-laying vertebrates) \\
\midrule
0 ($0\%$)   & \gen{6.8}{, I had a friend who used to teach high school English and he was like, "Oh, all you have to do is just get out there}  \\
%\midrule
%20  &  , most of these medals were named after the nation in which they were awarded. But our national identity is too strong. There's no more humility in \\
\midrule
40 ($0.009\%$)  & \gen{6.8}{ , many of these treasures were worth hundreds of thousands of dollars.\textbackslash n But this isn't the first time that a horse has been } \\
\midrule
60 ($0.015\%$)  &  \gen{6.8}{, through a freak occurrence, an invasion of house sparrows, which so often reduces the black-browed this nation recreats through} \\
\midrule
80 ($0.019\%$)  &  \gen{6.8}{, our own ancestors rode about on chicken-like air wings.\textbackslash n But this wonder of the air has no such wings.\textbackslash n Taking down} \\
\midrule
200 ($0.048\%$) &  \gen{6.8}{ of year, birds chase each and watching. flot racing form, bird, bird bird bird bird bird bird bird bird bird bird bird, Bird bird} \\
%{}&{}\\
%%\midrule
%%500 &  bird\%1:05:00 &  {\color{gray}Once upon a time} then bird\textbackslash n hollow lizard bird bird bird that bird song bird bird, bird bird bird bird bird bird bird bird bird bird bird bird bird. Bird Bird \\
%\toprule
% {} &        \hspace{-0mm}{\color{gray}Once upon a time}   {\small$+$} Generated induced for WordNet concept \href{\wordnet{bird}}{bird\%1:05:00}  \\
% \midrule
%200 &  \gen{6.8}{ of year, birds chase each and watching. flot racing form, bird, bird bird bird bird bird bird bird bird bird bird bird, Bird bird} \\

\bottomrule
\end{tabular}



\begin{tabular}{lp{13.5cm}}
{} & {} \\
 &        \hspace{-0mm}{\color{gray}Once upon a time}   {\small$+$} Generated induced for concept \href{\wordnet{lead}}{lead\%1:07:02} (an advantage held by a competitor in a race)  \\
\midrule
50 ($0.012\%$) &  \gen{6.8}{ the left-hander would always start at the front in the first two instances, but when Mauricio Gaponi rose to the podium,} \\

\bottomrule
\end{tabular}

\begin{tabular}{lp{13.5cm}}
{} & {} \\
 &        \hspace{-0mm}{\color{gray}Once upon a time}   {\small$+$} Generated induced for concept \href{\wordnet{lead}}{lead\%1:27:00} (a soft heavy toxic malleable metallic element)  \\
\midrule
100 ($0.024\%$) &  \gen{6.8}{Once upon a time a crust layer was applied to a partially fortified nickel base, thereby causing to zinc- and copper- ground element cob. The occurrence of those metal and chrome} \\
\bottomrule
\end{tabular}
%\begin{tabular}{llp{11cm}}
%\toprule
%K forced &         Concept & \hspace{-0mm}{\color{gray}Context} {\small$+$} Generated (induced for WordNet concept \href{\wordnet{bird}}{bird\%1:05:00})  \\
%\midrule
%0   &  \href{\wordnet{bird}}{bird\%1:05:00} & \gen{7.3}{\hspace{-0mm}{\color{gray}Once upon a time}, I had a friend who used to teach high school English and he was like, "Oh, all you have to do is just get out there}  \\
%%\midrule
%%20  &  \href{\wordnet{bird}}{bird\%1:05:00} &  \hspace{-0mm}{\color{gray}Once upon a time}, most of these medals were named after the nation in which they were awarded. But our national identity is too strong. There's no more humility in \\
%\midrule
%40  &  \href{\wordnet{bird}}{bird\%1:05:00} & \gen{7.3}{ \hspace{-0mm}{\color{gray}Once upon a time}, many of these treasures were worth hundreds of thousands of dollars.\textbackslash n But this isn't the first time that a horse has been a darling of} \\
%\midrule
%60  &  \href{\wordnet{bird}}{bird\%1:05:00} &  \gen{7.3}{\hspace{-0mm}{\color{gray}Once upon a time}, through a freak occurrence, an invasion of house sparrows, which so often reduces the black-browed this nation recreats through their} \\
%\midrule
%80  &  \href{\wordnet{bird}}{bird\%1:05:00} &  \gen{7.3}{\hspace{-0mm}{\color{gray}Once upon a time}, our own ancestors rode about on chicken-like air wings.\textbackslash n But this wonder of the air has no such wings.\textbackslash n Taking down} \\
%\midrule
%200 &  \href{\wordnet{bird}}{bird\%1:05:00} &  \gen{7.3}{\hspace{-0mm}{\color{gray}Once upon a time} of year, birds chase each and watching. flot racing form, bird, bird bird bird bird bird bird bird bird bird bird bird, Bird bird} \\
%%\midrule
%%500 &  bird\%1:05:00 &  {\color{gray}Once upon a time} then bird\textbackslash n hollow lizard bird bird bird that bird song bird bird, bird bird bird bird bird bird bird bird bird bird bird bird bird. Bird Bird \\
%\bottomrule
%\end{tabular}

}
%  \caption{Examples of generated sentences using GPT2-L with initial context {\color{gray}Once upon a time}, sorted by the number of top experts for WordNet concept \href{\wordnet{bird}}{bird\%1:05:00} forced. In parenthesis the percentage of experts forced out of the total 414720 units analyzed. The presence of the concept increases as we force more experts, empirically proving the impact of expert forcing on $p(y=c|x)$ in \eqref{eq:conditioned_gen}. The percentage of experts required is extremely low, saturating at 200 experts (0.048\%) in this example, where $p(y=c|x)$ already dominates $p(x)$ in \eqref{eq:conditioned_gen}.} 
    \caption{Examples of generated sentences using GPT2-L with initial context {\color{gray}Once upon a time}, sorted by the number of top experts for different WordNet concepts. In parenthesis the percentage of experts forced out of the total 414720 units analyzed. For concept  \href{\wordnet{bird}}{bird\%1:05:00}, the presence of the concept increases as we force more experts, empirically proving the impact of expert forcing on $p(y=c|x)$ in \eqref{eq:conditioned_gen}. The percentage of experts required is extremely low, saturating at 200 experts (0.048\%) in this example, where $p(y=c|x)$ already dominates $p(x)$ in \eqref{eq:conditioned_gen}. We also show generated sentences for concepts \href{\wordnet{lead}}{lead\%1:27:00 and lead\%1:07:02}, showing the model's ability to capture the meaning of the concept.} 
  \label{tab:generated_example}
\end{table*}


\subsection{Inducing concepts in Language Models}
\label{sec:generation}
%{\color{red}
%This section will contain examples of generated sentences for different concepts. If still space, a statistical analysis of the presence of concept as we force more top-K neurons. Which could be linked to \eq\eqref{eq:prob_gen} showing how $\pt(\G, \cG | \I)$ is proportional to K, or whatever relationship we find.
%}
Expert units can be used beyond model evaluation,. In this experiment, we use experts units for text generation.
The objective is threefold: (1) to demonstrate that ranking units by $\ap_c^m$ is a suitable strategy to find the experts for concept $c$; (2) to prove expert units are causal in the setting of LM, empirically showing that we can control $p(y=c|x)$ in \eq\eqref{eq:conditioned_gen}; and (3) to show that LMs can be conditioned without training or using additional parameters.  
\tabref\ref{tab:generated_example} illustrates the generation of sentences using GPT2-L while forcing the top-K experts for WordNet concept \href{\wordnet{bird}}{bird\%1:05:00}, as explained in \secref\ref{sec:forcing}. The decoding strategy is by nucleus filtering with $p=0.9$ \citep{Holtzman:ARXIV:2019}.  We observe how the presence of the concept gradually increases as we increase K, and that it saturates at about 200 experts forced. This result empirically explains \eq\eqref{eq:conditioned_gen}, showing that K controls $p(y=c|x)$ until saturation, when the effect of $p(x)$ (generate plausible sentences) is not evident anymore. The number of experts forced is extremely low, saturating at 200 experts (or 0.048\% of the 414720 units analyzed for GPT2-L), showing how LMs dedicate very selective units to specific concepts. This result draws a parallelism between the behavior of \TM and that of human brains \citep{Najafi:Neuron:2019}. Refer to \appref\ref{app:generation} for extended generation results.



%\paragraph{Experts per concept} In \fig\ref{fig:responsible_neurons} we show the histogram of expert units ($\map_c > 0.90$) per concept for RoBERTa-L. We observe that most of the concepts have less than 50 dedicated expert units (0.022\%), with a median of 7 experts (0.0032\%) per concept. Taking into account that 221184 units were analyzed for this model, we conclude that \TM dedicate very specific groups of experts to different concepts, and that these experts are actually causal as shown in \tabref\ref{tab:generated_example}.

%\begin{figure}[h]
%  \centering
%%\subfigure{ \includegraphics[width=\columnwidth]{images/responsible_neurons.pdf}}      
%  \begin{subfigure}[b]{\columnwidth}
%    \includegraphics[width=\textwidth]{images/responsible_neurons_roberta.pdf}
%%    \caption{Picture 1}
%%    \label{fig:1}
%  \end{subfigure}
%  \caption{
%  %Left: $\mmap$ as a function of the model size for different architectures. The measured $\mmap$ decreases linearly with the model size (note that the vertical axis is in log scale). Right: 
% Histogram of the number of expert units per \emph{sense} concept for model RoBERTa-L at $\map_c > 0.90$. The majority of concepts have less than 50 expert units associated, a very low value (0.022\%) compared to the 221184 units analyzed for RoBERTa-L showing that the number of experts per concept in a \oneTM is very selective. }\label{fig:responsible_neurons}
%\end{figure}
